Conditional Independence Testing for Random Objects via Generative Models

We propose a test of conditional independence for random objects taking values in metric spaces of negative type, allowing the conditioning variable to be either a random object or a high-dimensional vector. Our method uses multidimensional scaling and Nystr\"om extensions to obtain finite-dimensional representations of random objects from their pairwise distances, and generative neural networks to estimate conditional distributions in the embedded space. Samples from the fitted generators are then used to construct a doubly robust test statistic. Our main theoretical contribution is to quantify how errors from estimating and truncating the embeddings, together with errors in learning the conditional distributions, affect inference. We establish conditions under which these errors are asymptotically negligible, even when the embedding dimensions grow with the sample size. In particular, we derive explicit convergence rates when the conditional distributions admit generators with smooth, low-dimensional compositional structure. We establish asymptotic validity of the bootstrap test, consistency against fixed alternatives, and nontrivial power against local alternatives. Simulations with distribution-valued data demonstrate its competitive finite-sample performance.

==> supplement_labels.tex <==
\makeatletter
\@namedef{r@app:auxiliary-lemmas}{{K}{}}
\@namedef{r@app:proof-deep-approximation}{{H}{}}
\@namedef{r@app:proof-network-covering}{{F}{}}
\@namedef{r@app:proof-paper-mds}{{E}{}}
\@namedef{r@app:proof-paper-power}{{C}{}}
\@namedef{r@app:simulation-settings}{{J}{}}
\@namedef{r@app:vector-network-rates}{{I}{}}
\@namedef{r@eq:theory-boundary-noncentral-law}{{C-46}{}}
\@namedef{r@eq:theory-lowdim-exponential-choice}{{H-2}{}}
\@namedef{r@eq:theory-lowdim-polynomial-choice}{{H-1}{}}
\@namedef{r@item:paper-mds-population}{{i}{}}
\@namedef{r@lem:appendix-mercer}{{14}{}}
\@namedef{r@lem:centered-distance-kernel}{{13}{}}
\@namedef{r@lem:paper-mds-coordinate-identities}{{9}{}}
\@namedef{r@prop:paper-network-covering}{{2}{}}
\makeatother

